Premonition Net, A Multi-Timeline Transformer Network Architecture Towards Strawberry Tabletop Yield Forecasting

Yield forecasting is a critical first step necessary for yield optimisation, with important consequences for the broader food supply chain, procurement, price-negotiation, logistics, and supply. However yield forecasting is notoriously difficult, and oft-inaccurate. Premonition Net is a multi-timeline, time sequence ingesting approach towards processing the past, the present, and premonitions of the future. We show how this structure combined with transformers attains critical yield forecasting proficiency towards improving food security, lowering prices, and reducing waste. We find data availability to be a continued difficulty however using our premonition network and our own collected data we attain yield forecasts 3 weeks ahead with a a testing set RMSE loss of ~0.08 across our latest season.

==> Dockerfile <==
FROM archlinux:latest
# resetting all gnupg keys
RUN rm -rf /etc/pacman.d/gnupg && \
    pacman-key --init && \
    pacman-key --populate archlinux
# prepare pacman for use and generic dependencies
RUN pacman -Syyuu --noconfirm \
    archlinux-keyring \
    ca-certificates
RUN pacman-key --refresh-keys
# install specific dependencies we need
RUN pacman -S --noconfirm \
    biber \
    texlive-most \
    minted \
    which
# symlink biber from its strange path in /usr/bin/vendor_perl/biber to /usr/bin
RUN ln -s /usr/bin/vendor_perl/biber /usr/bin/biber
# copy all our files into the container ignoring .dockerignore'd files
COPY . /latex-src
# setting workdir to the src dir
WORKDIR /latex-src
# creating standard user to interact with files
RUN useradd archie && \
    chown -R  archie:archie /latex-src && \
    chmod 744 build.sh
USER archie
# setting default command to run if none given
CMD ["./build.sh"]


==> content/chapters/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio,angle=90]{people/George.jpg}}]{George Onoufriou}
% \begin{IEEEbiographynophoto}{George Onoufriou}
is a PhD student at the University of Lincoln, studying encrypted deep learning as part of a funded collaborative training partnership/ studentship. This studentship comes from the British Biotechnology and Biological Sciences Research Council in collaboration with Berry Gardens Growers, towards fruit yield forecasting. George is a cypherpunk, keenly interested in deep learning, privacy/ cryptography, (Arch) Linux, and open-source software in general. He is also founder of Deep Cypher Ltd., which seeks to enable and conduct encrypted deep learning as a service.
% \end{IEEEbiographynophoto}
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/mhanheide_2017_bw.png}}]{Prof. Marc Hanheide}
% \begin{IEEEbiographynophoto}{Dr Marc Hanheide}
is a Professor of Intelligent Robotics \& Interactive Systems in the School of Computer Science at the University of Lincoln, UK, and the director of the University’s cross-disciplinary research centre in Robotics, the Lincoln Centre for Autonomous Systems (L-CAS). He received the Diploma in computer science from Bielefeld University, Germany, in 2001 and the Ph.D. degree (Dr.-Ing.) also in computer science from Bielefeld University in 2006. From 2006 to 2009 he held a position as a senior researcher in the Applied Computer Science Group. From 2009 until 2011, he was a research fellow at the School of Computer Science at the University of Birmingham, UK.
Marc Hanheide is a PI in many national and international research projects, funded by H2020, EPSRC, InnovateUK, DFG, industry partners, and others, as well as the director of the EPSRC Centre for Doctoral Training (CDT) in Doctoral Training in Agri-Food Robotics (AgriFoRwArdS). The STRANDS, ILIAD, RASberry, and NCNR projects are among the bigger projects he is or was involved with. He features regularly in public media, has published more than 100 peer-reviewed articles, and is actively engaged in promoting the public understanding of science through appearances in dedicated events, media appearances, and public lectures.
% \end{IEEEbiographynophoto}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/TEDx_Leontidis.jpg}}]{Dr. Georgios Leontidis}
is the Director of the Interdisciplinary Centre for Data and AI, and a Reader in Machine Learning at the University of Aberdeen, UK, leading the Machine Learning group. Before joining the University of Aberdeen, Georgios was a Senior Lecturer at the University of Lincoln, UK. His expertise lies within the areas of Capsule Neural Networks, Domain Adaptation, and Self-Supervised Learning. Georgios has applied his research in different settings, including agri-food, gas turbines, nuclear reactors, environment, retail refrigeration systems, and healthcare. Georgios has been leading several projects, funded by industry, such as Siemens Energy and Tesco, EU-H2020, and UKRI. He is also a TEDx speaker and has featured in public media.
\end{IEEEbiography}
